Large Scale MRI Collection and Segmentation of Cirrhotic Liver

Liver cirrhosis represents the end stage of chronic liver disease, characterized by extensive fibrosis and nodular regeneration that significantly increases mortality risk. While magnetic resonance imaging (MRI) offers a non-invasive assessment, accurately segmenting cirrhotic livers presents substantial challenges due to morphological alterations and heterogeneous signal characteristics. Deep learning approaches show promise for automating these tasks, but progress has been limited by the absence of large-scale, annotated datasets. Here, we present CirrMRI600+, the first comprehensive dataset comprising 628 high-resolution abdominal MRI scans (310 T1-weighted and 318 T2-weighted sequences, totaling nearly 40,000 annotated slices) with expert-validated segmentation labels for cirrhotic livers. The dataset includes demographic information, clinical parameters, and histopathological validation where available. Additionally, we provide benchmark results from 11 state-of-the-art deep learning experiments to establish performance standards. CirrMRI600+ enables the development and validation of advanced computational methods for cirrhotic liver analysis, potentially accelerating progress toward automated Cirrhosis visual staging and personalized treatment planning.

==> takeout.tex <==


% \textbf{Cross-domain analysis:} Table~\ref{tab:crossdomain} shows results of segmentation networks pretrained on CirrMRI600$\rightarrow$T1W MRIs and tested on the part with CT scans pertaining to LiTS dataset. Results indicated that training pre-trained models with auto-configured architectures such as \textit{nnSynergyNet3D}, on the CirrMRI600$\rightarrow$T1W dataset improves generalization to liver CTs. This further provides valuable insight and promise towards building auto-configured synergistic models to be pre-trained on our proposed dataset. Such an approach could potentially reduce the workload of clinicians working on both CT and MRI modalities. %Future segmentation algorithms should focus on improving CT segmentation accuracy and better generalization across different imaging modalities.

% \begin{table*}[!t]
%     \caption{Cross-domain analysis of the model trained on \textbf{CirrMRI600+ $\rightarrow$T1W} and tested on LiTS. Bold shows the best performance while red is the second-best.} %~\cite{antonelli2022medical} CT dataset.
%     \centering
%     \footnotesize
%     \begin{adjustbox}{max width=\textwidth}
%     \begin{tabular}{lccccccc}
%         \toprule
%         \textbf{Method} & \textbf{mIoU} & \textbf{Dice} & \textbf{HD95} & \textbf{Precision} & \textbf{Recall} & \textbf{ASSD}  \\
%         \midrule
%         \texttt{nnUNet3D}~[\cite{isensee2021nnu}] & 80.02 & 81.19 & 29.78 & 80.98 & 83.21 & 6.52   \\
%          \texttt{nnFormer3D}~[\cite{zhou2023nnformer}] & \textcolor{red}{80.41} & \textcolor{red}{82.19} & \textcolor{red}{29.19} & \textbf{82.76} & \textcolor{red}{85.33} & \textcolor{red}{5.91}   \\
%          \texttt{TransUNet3D}~[\cite{chen2021transunet}] & 76.87 & 77.89 & 33.78 & 78.87 & 80.02 & 7.08  \\
%          \texttt{SwinUNITR}~[\cite{hatamizadeh2021swin}] & 78.89 & 79.12 & 30.98 & 77.98 & 80.03 & 6.67   \\
%          \texttt{TransBTS}~[\cite{wenxuan2021transbts}] & 79.11 & 81.11 & 29.48 & 79.91 & 81.19 & 6.01   \\
%          \texttt{nnSynergyNet3D}~[\cite{gorade2024synergynet}] & \textbf{81.88} & \textbf{83.38} & \textbf{29.01} & \textcolor{red}{81.15} & \textbf{86.02} & \textbf{5.55}  \\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{tab:crossdomain}
% \end{table*}
